MM2RTB: Bringing Multimedia Metrics to Real-Time Bidding

In display advertising, users' online ad experiences are important for the advertising effectiveness. However, users have not been well accommodated in real-time bidding (RTB). This further influences their site visits and perception of the displayed banner ads. In this paper, we propose a novel computational framework which brings multimedia metrics, like the contextual relevance, the visual saliency and the ad memorability into RTB to improve the users' ad experiences as well as maintain the benefits of the publisher and the advertiser. We aim at developing a vigorous ecosystem by optimizing the trade-offs among all stakeholders. The framework considers the scenario of a webpage with multiple ad slots. Our experimental results show that the benefits of the advertiser and the user can be significantly improved if the publisher would slightly sacrifice his short-term revenue. The improved benefits will increase the advertising requests (demand) and the site visits (supply), which can further boost the publisher's revenue in the long run.

==> backup.tex <==
\begin{table}[t]
\small
\centering
\caption{Summary of key notations.}
\label{tab:notations}
\vspace{-7pt}
\begin{tabular}{r|p{2.75in}}
\hspace{-20pt} Notation \hspace{-5pt} & Description\\
\hline
$W$ & Set of webpages of the publisher\\
$A_w$  & Set of ad slots on webpage $w \in W$\\
%$A_w$  & Set of auctions for a user's visit at webpage $w \in W$\\
$N_{a,w}$   & Set of advertisers in the auction for ad slot $a \in A_w$\\
$K$     & Set of metric variables in the trade-offs optimization, $|K| = 6$\\
$b_{i,a,w}$ & Bid price of advertiser $i$ in the auction for slot $a$, $i \in N_{a,w}$\\
$b_{(i),a,w}$ & $i$th highest bid in auction $a$, $i \in N_{a,w}$\\
$y_{i,j,a,w}$ & Probability that advertiser $i$ is allocated to slot $j$ in auction $z$\\
$p_{i,z}(b_z)$ & Payment of advertiser $i$ in auction $z$, $b_z=(b_{1,z}, \cdots, b_{n_z,z})$\\
$\omega_k$ & Weight of variable $k$ in the re-ranking, $k \in K$\\
$x_{k,*,z}$ & Value of variable $k$ for the selected advertiser in auction $z$ by our proposed model\\
$x_{k,\neg,z}$ & Value of variable $k$ for the selected advertiser in auction $z$ by the SP auction (the ground truth)\\
$\xi_{k,Z}$ & Average change of value for variable $k$ of auctions in set $Z$\\
$\theta_k$ & Threshold for the change of value for variable $k$\\
$rs_{i,z}$ & Rank score of advertiser $i$ in auction $z$\\
$rs_{*,z}$ & Rank score of the selected advertiser in auction $z$ by our proposed model\\
$rs_{\neg,z}$ & Rank score of the selected advertiser in auction $z$ by the SP auction (the ground truth)\\
\end{tabular}
\end{table}



\begin{table}[t]
\footnotesize
\centering
\caption{Multimedia datasets. The crawler type I collect webpages as many as possible from a seed URL and the crawler type II repeatedly accesses to a set of particular webpages. }
\label{tab:multimedia_datasets}
\vspace{-7pt}
\begin{tabular}{r|r|r|r|r|r}
\hline
\multicolumn{2}{r|}{Platform} & Yahoo & Yahoo & MSN & MSN \\
\hline
\multicolumn{2}{r|}{Crawler type} & I & II & I & II \\
\multicolumn{2}{r|}{From} & \hspace*{-2pt} 20 Jan 2017 & \hspace*{-2pt} 20 Jan 2017 & \hspace*{-2pt}  20 Jan 2017 & \hspace*{-2pt}  20 Jan 2017\\
\multicolumn{2}{r|}{To}   & \hspace*{-2pt} 30 Jan 2017 & \hspace*{-2pt} 30 Jan 2017 & \hspace*{-2pt} 30 Jan 2017 & \hspace*{-2pt} 30 Jan 2017\\
\multicolumn{2}{r|}{Location} & Singapore & Singapore & Singapore & Singapore\\
\multicolumn{2}{r|}{\# of webpages} & & & &\\ 
\multicolumn{1}{r}{}  & with 1 slot  & 1481 & 1909 & 798 & 686\\
\multicolumn{1}{r}{}  & with 2 slots & 1978 & 3510 & 1519 & 3689\\
\multicolumn{1}{r}{}  & with 3 slots & 1173 & 4329 & 3633 & 146\\
\multicolumn{1}{r}{}  & with $\geq 4$ slots & 1599 & 2468 & 41 & 241\\
\multicolumn{2}{r|}{\# of total impressions} & 15836 & 31951 & 14899 & 9466\\
\multicolumn{2}{r|}{\# of unique advertisers} & 692 & 631 & 160 & 163\\
\hline
\end{tabular}
\vspace{10pt}
\caption{Ad auction datasets.}
\vspace{-7pt}
\label{tab:auc_datasets}
\begin{tabular}{r|r|r}
\hline
Dataset & SSP & Microsoft\\ 
\hline
Ad type    & Display  & Search\\
Ad auction & SP (RTB) & GSP   \\
Market  & UK & US\\

[From, To]  & [08 Jan 2013, 14 Feb 2013] & [26 Dec 2011, 03 Mar 2012]\\
\# of ad slots      & 31 & 4,376      \\
\# of user tags     & NA & NA        \\
\# of publishers    & NA & 1 \\
\# of bidders       & 374      & NA\\ 
\# of auctions      & 6,646,643  & 35,550\\ 
\# of bids          & 33,043,127 & NA\\
Bid quote               & GBP/CPM  & GBP/CPC\\
Bids of each auction & $\surd$ & NA\\
Winning bid          & $\surd$ & $\surd$\\
Winning payment      & $\surd$ & $\surd$\\
Estimated CTR        & NA      & $\surd$\\
\hline
\end{tabular}
\vspace{10pt}
\caption{Summary of CTRs in the Microsoft dataset.}
\label{tab:microsoft_dataset}
\vspace{-7pt}
\begin{tabular}{r|r|r|r|r}
\hline
Position & Minimum of CTR & Maximum of CTR & Mean of CTR & Std. of CTR \\
\hline
1  &     0.00\textperthousand  & 333.30\textperthousand  &   13.97\textperthousand & 28.49\textperthousand  \\
2  &     0.00\textperthousand  & 200.00\textperthousand  &   7.97\textperthousand  & 15.30\textperthousand  \\
3  &     0.00\textperthousand  & 750.00\textperthousand  &   5.66\textperthousand  &  12.47\textperthousand \\
4  &     0.00\textperthousand  & 90.90\textperthousand   &   4.53\textperthousand  &  9.68\textperthousand  \\
5  &     0.00\textperthousand  & 76.90\textperthousand   &   1.53\textperthousand  &  3.58\textperthousand  \\
6  &     0.00\textperthousand  & 333.30\textperthousand  &   1.11\textperthousand  &  3.62\textperthousand  \\
7  &     0.00\textperthousand  & 1000.00\textperthousand &   0.68\textperthousand  &  5.73\textperthousand  \\
8  &     0.00\textperthousand  & 108.10\textperthousand  &   0.51\textperthousand  &  1.65\textperthousand  \\
\hline
\end{tabular}
\end{table}

\begin{algorithmic}[0]
\State \textbf{Step 1: Sampling an auction in RTB:}\\ 
We randomly sample an auction from the SSP dataset. The auction contains a set of advertisers and their bids. 

\State \textbf{Step 2: Creating the ground truth data}\\
Since the given webpage has an ad displayed when it is web crawled. This original ad is considered as the ground truth. 

\State \textbf{Step 3: Sampling candidate ads:}\\ 
Let $n$ denote the number of advertisers in the sampled auction in Step 1. We then randomly sample $n-1$ ads from the same multimedia dataset of the webpage. To ensure the uniqueness of each ad in the auction, we exclude the original ad when we sample $n-1$ ads from the multimedia dataset. 

\State \textbf{Step 4: Matching ads and bids:}\\ We match the $n$ bids with $n$ ads. Since the original ad is displayed, we consider it belongs to the winning advertiser in the auction and match it with the highest bid. The rest $n-1$ ads and $n-1$ bids are then randomly matched. 

\State \textbf{Step 5: Simulating CTRs:}\\ For each ad, we generate its CTR from a uniform distribution in the range of 0 and 13.97\textperthousand $+$ 1.96 $\times$ 28.49\textperthousand. This is based on the mean and std. of CTRs in the first position in the Microsoft dataset, as also shown in Table~\ref{tab:microsoft_dataset}.
\end{algorithmic}

% \begin{table*}[tp]
% \small
% \centering
% \caption{Specifications of metric variables for Stage II.}
% \label{tab:second_stage_var_spec}	
% \vspace{-7pt}
% \begin{tabular}{l|l|l|l|l}
% \hline
% \multirow{2}{*}{Variable}   & \multicolumn{3}{c|}{Computation} & \multirow{2}{*}{Input for Stage II}\\
% \cline{2-4}
%           & Method & Input & Output         & \\
% \hline
% Publisher's revenue    & Stage I       & Bid & Payment & $x_{1,i,z} = $ normalized $p_{i,z}$\\
% Advertiser's utility    & Stage I      & Bid, payment & Utility    & $x_{2,i,z} = $ normalized $(v_{i,z} - p_{i,z})$\\
% Ad memorability & MemNet~\cite{khosla2015understanding} & Ad image & Memorability score & $x_{3,i,z} = $ normalized score\\
% Ad CTR    & Given by data         & CTR &  CTR & $x_{4,i,z} = $ normalized CTR\\
% Contextual relevance & TakeLab~\cite{vsaric2012takelab} & Title, keywords, description & Semantic similarity score & $x_{5,i,z} = $ normalized score\\
% Ad saliency & MBS~\cite{zhang2015minimum} & Web page snapshot, ad image & Saliency map and ratio & $x_{6,i,z} = $ normalized ratio \\
% \hline 
% \end{tabular}
% \end{table*}

